Abstract Fixpoint Computations with Numerical Acceleration Methods

Static analysis by abstract interpretation aims at automatically proving properties of computer programs. To do this, an over-approximation of program semantics, defined as the least fixpoint of a system of semantic equations, must be computed. To enforce the convergence of this computation, widening operator is used but it may lead to coarse results. We propose a new method to accelerate the computation of this fixpoint by using standard techniques of numerical analysis. Our goal is to automatically and dynamically adapt the widening operator in order to maintain precision.

==> interval_domain.tex <==
In this section, we adapt the \textit{Shanks Transformation} presented
in Section~\ref{sec:acceleration-of-convergence} to the interval
domain.

The interval domain \cite{CousotCousot77-1} is an abstraction of a set
of values represented by the minimum and the maximum values of this
set. The lattice operations over intervals is given in the
Figure~\ref{fig:lattice-and-arithmetic-operations-over-intervals}.

\begin{figure}[ht]
  \centering
  \begin{align*}
    [a_1,b_1] \sqsubseteq [a_2,b_2] & \Leftrightarrow a_1 \geq
    a_2 \cap b_1 \leq b_2
    \\
    \bot & = [a, b]\quad\text{such as } a > b
    \\
    \top & = [-\infty,\quad +\infty]
    \\
    [a_1,b_1] \sqcup [a_2,b_2] & \Leftrightarrow [\min(a_1 + a_2),\quad
    \max(b_1 + b_2)]
    \\
    [a_1,b_1] \sqcap [a_2,b_2] & \Leftrightarrow [\max(a_1 + b_2),\quad
    \min(b_1 + a_2)]
    \\
    [a_1, b_1] \nabla [a_2, b_2] & 
    \Leftrightarrow 
    \left[
      \begin{cases}
        a_1 & \mbox{if } a_1 \leq a_2
        \\
        -\infty& \mbox{otherwise}
      \end{cases}
      ,\quad
      \begin{cases}
        b_1 & \mbox{if } b_1 \geq b_2
        \\
        +\infty& \mbox{otherwise}
      \end{cases}
    \right]  
    \\
    [a_1,b_1] + [a_2,b_2] & \Leftrightarrow [a_1 + a_2,\quad
    b_1 + b_2]
    \\
    [a_1,b_1] - [a_2,b_2] & \Leftrightarrow [a_1 + b_2,\quad
    b_1 + a_2]
    \\
    [a_1,b_1] \times [a_2,b_2] & \Leftrightarrow
    \left[\min\left(a_1a_2, a_1b_2 , b_1a_2, b_1b_2\right),\right.
    \\
    &
    \qquad
    \left.\max\left(a_1a_2, a_1b_2, b_1a_2, b_1b_2\right)\right]
    \\
    [a_1,b_1] \div [a_2,b_2] & \Leftrightarrow \left[\frac{a_1}{b_2},\quad
    \frac{b_1}{a_2}\right]\quad\text{with } 0\not\in [a_2,b_2]
  \end{align*}
  \caption{Lattice and arithmetic operations over intervals}
  \label{fig:lattice-and-arithmetic-operations-over-intervals}
\end{figure}

\begin{example}
  
\end{example}

